A Search for Transit Duration Variations in M dwarf Multi-Planet Systems

The nominal habitable zone for exoplanets orbiting M dwarfs lies close to the host star, making dynamical considerations especially important. One consequence of this proximity is the expectation of spin synchronization, with implications for atmospheric circulation. Several mechanisms can maintain non-zero obliquities over long timescales in compact multi-planet systems, including capture into Cassini State 2 (CS2) and other forms of secular spin-orbit coupling; such pathways are plausible in the orbital architectures of close-in M-dwarf planets. In this study, we search for transit duration variations (TDVs) consistent with the nodal precession rates predicted by Laplace-Lagrange secular theory in compact M-dwarf multi-planet systems. Our sample includes 23 exoplanets orbiting 12 stars. We compare recent, high-precision transit durations obtained from JWST white-light curves with measurements published at the discovery epoch and afterward. The resulting transit duration variation ranges from seconds to minutes, and we fit a linear trend to duration versus time for each planet. All systems are consistent with flat (no TDV) at the 3{\sigma} level. The strongest candidate is TRAPPIST-1d, whose fitted slope differs from zero with 2.2{\sigma} confidence. We calculate the expected TDV signals predicted by secular precession and compare them to the observed limits. Our null detection is consistent with the low-impact-parameter regime, where theoretical TDVs are only a few seconds per decade and below our sensitivity. Higher-impact-parameter configurations predict substantially larger TDVs and are disfavored: under uniformly distributed geometries, at least half of the allowed configurations would be excluded.

==> extra_text.tex <==
After the production of white light curve, linear de-trending of the observed flux was done. Linear trend with negative slope in the obtained white light curve is a typical JWST readout patter. Therefore, depending on which package to use for MCMC fitting and visualization of best-fit model, the linear de-trending is necessary. Since we utilized python package \textit{batman} \citep{kreidberg_batman_2015}, linear de-trending was necessary. The off-transit normalized flux were extracted for each planet's white light curve sample, performing polynomial fitting using python package \textit{numpy.polyfit} with degree of 2 as a linear de-trending function, and dividing the original white light curve with the obtained polynomial function. The uncertainty of flux value was also obtained after this linear de-trending, compensating the effect by JWST readout patter, by computing the uncertainty of off-transit flux values. The linear de-trending enables us to calculate mean flux values with higher precession when calculating the uncertainty of the flux values. This process is crucial for white light curve fitting as to constrain best-fit model in higher fidelity.
Here, we represent 2 simultaneous transiting events observed by JWST, which are Trappist-1b and Trappist-1c, and TOI-270b and TOI-270d. The details of extracting the orbital parameters of planets simultaneously in a single transit visit for both of the planetary systems is described in Section 3.
 
 A science product after JWST stage 1 pipeline, rateints.fits file, were downloaded for each sample from MAST online Archive that is open to public. Data reduction process after stage 1 JWST pipeline was done by the individual pipeline inspired by Nikolov et al. 2020, which can be found through STScI's JWebinnar page open to public. The data reduction process resembles stage 2 JWST pipeline. This includes 1/f correction, assigning World Coordinate Systems (WCS), bad pixel replacement, spectral tracing and extraction of 1D data from 2D data. However, flat fielding and photoelectric effect are skipped in the pipeline although it does not show any systematic error but rather a random error in the obtained transit duration values for each planet. More details on JWST stage 1 and stage 2 data product can be found in JWST webpage \citep{bushouse_jwst_2025}. White light curve was produced by data from nrs1 detector for each data. The rateints.fits data consisted of multiple segments, each dividing the observation time to some extent. We therefore integrated multiple segments into one for each data respectively while ensuring that the integration number and observation time is in linear relation. Although G395H, G395M, and G235H dispersers have another detector, nrs2, which covers wavelength region of around 3.8$\mu$m to 5.2$\mu$m, we did not utilize them for data analysis. Two distinctive detectors play a vital role for producing transmission spectra for different wavelength coverage as it holds information of specific absorption line created by its corresponding molecules. However, we aim to obtain only the transit duration. Therefore, we excluded the data from nrs2.

The initial rateints.fits file is in 3D structure, x-axis containing wavelength information y-axis containing spatial information, and z-axis containing time. White light curve production focuses mainly on reducing wavelength and spatial information. The rateint.fits data consists of multiple segments, dividing the observation time into 2 or 3 depending on the data. Therefore, after assigning WCS, we integrated each segments into one, ensuring that the integration number and observation time is in linear relationship. The wavelength coverage of nrs1 detector alongside the type of optical element are as follows: PRISM;CLEAR: 0.60$\mu$m $\sim$ 5.30$\mu$m, G395H;F290LP: 2.87$\mu$m $\sim$ 3.69$\mu$m, G235H;F170LP: 1.66$\mu$m $\sim$ 2.18$\mu$m, G395M;F290LP: 2.87$\mu$m $\sim$ 5.10$\mu$m. 1/f correction is a peculiar noise which can be seen in any JWST data, which is the noise in vertical direction. Since there contains bad pixels, this can be from either cosmic rays or dead pixels although dead pixels make up the majority, we therefore identify the peak of the DN/s for each x-axis, and fit a nominal point spread function (PSF) profile. The bad pixels are then replaced by the values obtained from the PSF profile if the difference in the observed data and PSF profile is outside 3$\sigma$. Spectral tracing is done by fitting the maximum DN/s pixel with polynomial function. We then extract the light count for each x-axis by integrating from the maximum count until 3 pixels away from the maximum. Therefore, we obtain 1D data from the 2D data. More details on the data reduction process is described in the code availability section.

Although we constructed our sample to overlap as much as possible with the theoretically predicted TDV distribution (see Figure \ref{fig:theoreticalcomparison}), our JWST search also retrieved planets orbiting M dwarfs that do not appear in the catalog of \citet{Guerrero2025}. Their absence from that catalog does not imply that TDVs cannot be detected in those systems. Instead, these planets were originally discovered via radial-velocity (RV) observations and lack the full set of transit geometry parameters required for forward modeling of TDVs.


The selection of samples for data analysis relied on two factors (1): Planets in M dwarf multi-planet systems with observable transit duration variation (TDV's) target stated in (Guerrero et al, 2025) (2): Data availability of JWST observation in MAST online archive out in public. In total, we analyzed 12 M dwarf multi-planet systems, comprised of 23 transiting planets which were available in MAST online archive. The analyzed samples are summarized in table \ref{table:planetsample}. Although we assembled our data samples to match the theoretically predicted TDV distributions (see fig \ref{fig:theoreticalcomparison}), we also obtained transit duration values for several planets orbiting M-dwarf stars that did not appear in the sample compiled by (Guerrero et al. 2025). The absence of these planets in their catalog does not imply that TDVs cannot be detected for them. Rather, these systems were originally discovered through radial-velocity measurements and lack sufficient parameter information to compute TDVs. 

Exoplanet orbiting M dwarf stars, half the mass of the Sun or smaller, will become the primarily exoplanet studies in the next decade. Recent research in exoplanet has established a strong foundation in looking for Earth-like planets, namely rocky planets, and the abundance of such planetary systems in the Milky Way galaxy. Moreover, the advent of James Webb Space Telescope (JWST; \cite{2006SSRv..123..485G}) has captivated us with its capability of studying such planets, once we thought was too difficult. JWST enabled us to focus on the atmospheric characterization of planet orbiting M dwarf stars (e.g. \cite{2023ApJ...956L..13M}; \cite{2024arXiv240303325B}) with the highest fidelity every. These background have opened a completely new window of considering habitability of exoplanets orbiting around M dwarf stars.

The research objective is to verify whether planets in M-dwarf multi-planet systems that are captured in Cassini state 2 can sustain high obliquity states and exhibit rapid orbital precession. This orbital mechanics prevents those planets from being in tidally locked state due to the proximity to its host star, having a day-night cycle while maintaining high obliquity. This has an implication to habitability of exoplanets orbiting M-dwarf stars. Rapid orbital precession indicates oscillation in orbital plane of a planet, which results in change of transit duration over time. We therefore aim to measure such phenomenon by measuring the transit duration by using the most recent JWST observation considering its high S/N, and by comparing previous results of such values in M dwarf multi-planet system since its discovery epoch. We then compare our obtained results with the theoretical predictions \citep{2024ESS.....561610G}, of which to what extent the change in transit duration is plausible to be measured during the span between the discovery epoch and recently observed date, discussing the orbital mechanics that might dominate other then Cassini State 2 if the results were inconsistent with the predictions. 

Most importantly, the plausibility of planets excited into second Cassini State is the highest in those orbiting M dwarfs, hence adds the significance of studying M dwarfs. The tendency of M dwarfs to host compact systems of many planets heightens the likelihood further. While excitation into Cassini States is likely for close-in planetary systems generally \citep{2020AAS...23524905M};\citep{2022MNRAS.509.3301S}, the existence of more than two planets orbiting the star enhances the production of oblique planets via the Cassini State phenomenon\citep{Millholland_2019}. It is this phenomenon that we propose to investigate: the planets capture into Cassini State 2 of temperature planets orbiting small stars, via a specific dynamical marker, orbital precession. 
